A Deep Neural Network Sentence Level Classification Method with Context Information

In the sentence classification task, context formed from sentences adjacent to the sentence being classified can provide important information for classification. This context is, however, often ignored. Where methods do make use of context, only small amounts are considered, making it difficult to scale. We present a new method for sentence classification, Context-LSTM-CNN, that makes use of potentially large contexts. The method also utilizes long-range dependencies within the sentence being classified, using an LSTM, and short-span features, using a stacked CNN. Our experiments demonstrate that this approach consistently improves over previous methods on two different datasets.

==> relaWork.tex <==
\section{Related work}

%Until 2011 vanilla feedforward neural network with carefully manully selected feature input (e.g. stop words filter,
%tfidf, parse tree) \cite{Wiener1995,Ruiz2002,Wang2009,Harrag2010,Zheng2012} were main steam of ANN text classification
%reaserch. In 2011 \newcite{Collobert2011} argue apply word embedding and convolutional neural network able to perform
%better than vanilla feedforward neural network with feature selection. This approach soon been adopated in text
%classification task by later researches \cite{Kim2014,Conneau2017}.
%

Since their introduction \cite{Collobert2011}, CNNs with word
embedding language models have become common for text classification tasks \cite{Kim2014,Conneau2017}.
One limitation of the original CNN approach is the loss of long distance dependencies. 
In order to deal with this in image and speech recognition tasks,
\newcite{Xu2015,Sainath2015} combined CNNs with a Recurrent Neural
Network (RNN) layer. \newcite{Zhou2015} subsequently applied this to text classification.
However, the CNN-RNN approach was originally devised for sequence
labelling, is biased towards later words in the sequence,
and does not perform better than CNN alone. \newcite{Huynh2016} suggested reversing the architecture to first 
apply the RNN followed by a CNN with pooling to obtain global features. This gave results that improved 
over CNN-RNN, but not over CNN alone. 
In this paper, we build on \newcite{Huynh2016}'s approach by replacing the GRU-based RNN \cite{Cho2014} with an LSTM \cite{Hochreiter1997} and 
by using multiple kernel 
sizes and more features in the subsequent CNN layer.

\newcite{Lee2016} showed that when classifying short texts, accuracy can be
boosted by adding a CNN or LSTM derived vector representation of the
surrounding context. For long contexts (such as patient records which
may include well over 100 sentences), however, this will incur a significant additional
computational cost. In this paper, we therefore apply an adaptation of the
FOFE encoding \cite{Zhang2015} to encode context.


